Theoretical Analysis and Evaluation of NoCs with Weighted Round-Robin Arbitration

Fast and accurate performance analysis techniques are essential in early design space exploration and pre-silicon evaluations, including software eco-system development. In particular, on-chip communication continues to play an increasingly important role as the many-core processors scale up. This paper presents the first performance analysis technique that targets networks-on-chip (NoCs) that employ weighted round-robin (WRR) arbitration. Besides fairness, WRR arbitration provides flexibility in allocating bandwidth proportionally to the importance of the traffic classes, unlike basic round-robin and priority-based arbitration. The proposed approach first estimates the effective service time of the packets in the queue due to WRR arbitration. Then, it uses the effective service time to compute the average waiting time of the packets. Next, we incorporate a decomposition technique to extend the analytical model to handle NoC of any size. The proposed approach achieves less than 5% error while executing real applications and 10% error under challenging synthetic traffic with different burstiness levels.

==> acronyms.tex <==
\newacronym{TDP}{TDP}{thermal design power}
\newacronym[longplural={general-purpose processors}]{GPP}{GPP}{general-purpose processor}
\newacronym[longplural={no-operations}]{NOP}{NOP}{no-operation}
\newacronym{ILP}{ILP}{instruction-level parallelism}
\newacronym{VLIW}{VLIW}{very long instruction word}
\newacronym{DVFS}{DVFS}{dynamic voltage and frequency scaling}
\newacronym{DVS}{DVS}{dynamic voltage scaling}
\newacronym{DMR}{DMR}{dual modular redundancy}
\newacronym{HPC}{HPC}{high-performance computing}
\newacronym{DWC}{DWC}{duplication with comparison}
\newacronym{TMR}{TMR}{triple modular redundancy}
\newacronym{ROB}{ROB}{re-order buffer}
\newacronym{DSE}{DSE}{design space exploration}
\newacronym{TSH}{TSH}{tricriteria scheduling heuristics}
\newacronym{PG}{PG}{power gating}
\newacronym{CG}{CG}{clock gating}
\newacronym[longplural={functional units}]{FU}{FU}{functional unit}
\newacronym{PC}{PC}{program counter}
\newacronym{ECC}{ECC}{error correction code}
\newacronym[longplural={basic blocks}]{BB}{BB}{basic block}
\newacronym{BBHT}{BBHT}{basic block history table}
\newacronym{ASIC}{ASIC}{application-specific integrated circuit}
\newacronym{CMOS}{CMOS}{complementary metal-oxide-semiconductor}
\newacronym{ADPCM}{ADPCM}{adaptive differential pulse-code modulation}
\newacronym{DFT}{DFT}{discrete Fourier transform}
\newacronym{AVF}{AVF}{architectural vulnerability factor}
\newacronym{RTL}{RTL}{register-transfer level}
\newacronym{SET}{SET}{single-event transient}
\newacronym{SEU}{SEU}{single-event upset}
\newacronym{SBU}{SBU}{single bit upset}
\newacronym{MBU}{MBU}{multiple bit upset}
\newacronym[longplural={arithmetic logic units}]{ALU}{ALU}{arithmetic logic unit}
\newacronym{MMX}{MMX}{multimedia extension}
\newacronym{LUDCMP}{LUDCMP}{LU decomposition}
\newacronym{EDFP}{EDFP}{energy-delay-failure product}
\newacronym{EDP}{EDP}{energy-delay product}
\newacronym{ISA}{ISA}{instruction set architecture}
\newacronym{TCL}{TCL}{tool command language}
\newacronym{SEE}{SEE}{single-event effect}
\newacronym{DCT}{DCT}{discrete cosine transform} 
\newacronym{TLP}{TLP}{thread-level paralellism}
\newacronym{SRAM}{SRAM}{static random access memory}
\newacronym{FPGA}{FPGA}{field-programmable gate array}
\newacronym{ABFT}{ABFT}{algorithm-based fault tolerance}
\newacronym{TID}{TID}{total ionizing dose}
\newacronym{NMR}{NMR}{N-modular redundancy}
\newacronym{OoO}{OoO}{out-of-order}
\newacronym{VHDL}{VHDL}{VHSIC hardware description language}
\newacronym{DWP}{DWP}{duplicate when possible}
\newacronym{LANSCE}{LANSCE}{Los Alamos Neutron Science Center}
\newacronym{ACE}{ACE}{architecturally correct execution}
\newacronym{PPI}{PPI}{parallel programming interface}
\newacronym{OpenMP}{OpenMP}{open multi processing}
\newacronym{Pthreads}{Pthreads}{POSIX threads}
\newacronym{MPI}{MPI}{message passing interface}
\newacronym{FIFO}{FIFO}{first-in-first-out}
\newacronym{GCC}{GCC}{GNU compiler collection}
\newacronym{RAW}{RAW}{read after write}
\newacronym{MWPUETF}{MWPUETF}{mean work per unit of energy to failure}
\newacronym{MWTF}{MWTF}{mean work to failure}
\newacronym{LUT}{LUT}{look-Up table}
\newacronym{MITF}{MITF}{mean instructions to failure}
\newacronym{NASA}{NASA}{National Aeronautics and Space Administration}
\newacronym{CPU}{CPU}{central processing unit}
\newacronym{CFG}{CFG}{control flow graph}
\newacronym{MCCP}{MCCP}{multiple clustered core processor}
\newacronym{RMT}{RMT}{redundant multithreading}
\newacronym{IPC}{IPC}{instructions per cycle}
\newacronym{PID}{PID}{process ID}
\newacronym{DPM}{DPM}{dynamic power management}
\newacronym{MLP}{MLP}{multi-layer perceptron}
\newacronym{IPS}{IPS}{instructions per second}
\newacronym{NN}{NN}{neural network}
\newacronym{RC}{RC}{reconfiguration controller}
\newacronym{ML}{ML}{machine learning}
\newacronym{IL}{IL}{imitation learning}
\newacronym[longplural={systems-on-chip}]{SoC}{SoC}{system-on-chip}
\newacronym{WiFi-TX}{WiFi-TX}{WiFi transmitter}
\newacronym{WiFi-RX}{WiFi-RX}{WiFi receiver}
\newacronym{Range-Det}{Range-Det}{range detection}
\newacronym{SCT}{SCT}{single carrier transmitter}
\newacronym{SCR}{SCR}{single carrier receiver}
\newacronym{RT}{RT}{real-time}
\newacronym{RL}{RL}{reinforcement learning}
\newacronym{PMU}{PMU}{performance monitoring unit}
\newacronym{DAG}{DAG}{directed acyclic graph}
\newacronym{PAPI}{PAPI}{performance application programming interface}



==> algorithms/dagger.tex <==
\begin{algorithm}[tb]
\footnotesize
% \small
\SetNoFillComment
\caption{Methodology to aggregate data in a hierarchical imitation learning framework}
\label{algo:dagger}
\SetAlgoLined
\For {task T $\in \mathcal{T}$} {
$s$ = Get current state for task T \\
% $C_{i}$ = Assign cluster using IL policy for task T \\
\If {$\pi_{C}(s)$ == $\pi_{C}^*(s)$} {
    % $PE_{i}$ = Assign PE within cluster $C_{i}$ \\
    \If {$\pi_{P,c}(s)$ != $\pi_{P,c}^*(s)$} {
        Aggregate state $s$ and label $\pi_{P,c}^*(s)$ to the dataset
    }
}
\Else {
    Aggregate state $s$ and label $\pi_{C}^*(s)$ to the dataset \\
    $c^{*}$ = $\pi_{C}^*(s)$ \\
    \If {$\pi_{P,c^*}(s)$ != $\pi_{P,c^{*}}^*(s)$} {
        Aggregate state $s$ and label $\pi_{P,c}^*(s)$ to the dataset
    }
}
% Assign T to PE $\pi_{P,c}(s)$
\tcc{\textbf{Assign T to the predicted PE}}
}
\end{algorithm}

==> algorithms/dagger_2.tex <==
\begin{algorithm}[tb]
\footnotesize
\SetNoFillComment
\caption{Hierarchical Imitation Learning Framework \todo{Option 2 - remove Algorithm 1 and Algorithm 2 and only keep this one (merged version)}} \label{algo:dagger}
\SetAlgoLined
\ForEach {task i in list\_of\_tasks $L$} {
$\mathcal{S}(i)$ = Get current state  \\
\tcc{\textbf{Level 1 - cluster selection}}
$C_i$ = $\bm{\pi_{C}}(\mathcal{S}(i))$ \\
\If {$C_i$ matches the Oracle decision $C_i^{*}$} {
    /* Proceed with execution */
}
\Else {
    Aggregate state $\mathcal{S}(i)$ and label $C_i^{*}$ to the dataset \\
}
\tcc{\textbf{Level 2 - PE selection}}
$\pi_{PE_{C}}$ $\leftarrow$  select the $\pi_{PE}$ of cluster $C_i$ \\
$PE_i$ = $\bm{\pi_{PE_{C}}}(\mathcal{S}(i))$ \\
\If {$PE_i$ matches the Oracle decision $PE_i^{*}$} {
    /* Proceed with execution */
}
\Else{
    Aggregate state $\mathcal{S}(i)$ and label $PE_i^{*}$ to the dataset \\
}
Assign task $i$ to $PE_i$
% t.PE $\leftarrow$ $PE_i$ 
}
\end{algorithm}

==> algorithms/hierarchical.tex <==
\begin{algorithm}[tb]
\footnotesize
% \small
\SetNoFillComment
\caption{Hierarchical imitation learning Framework}
\label{algo:hierarchical}
\SetAlgoLined
\For {task T $\in \mathcal{T}$} {
% ${s}(i)$ = $\pi_{C}(\mathcal{F},T)$ /*Get current state */ \\
$s$ = Get current state for task T \\
\tcc{\textbf{Level-1 IL policy to assign cluster}}
% $\mathcal{S}(t)$ = Get current state  \\
$c$ = $\pi_{C}(s)$ \\
\tcc{\textbf{Level-2 IL policy to assign PE}}
p = $\pi_{P,c}(s)$ \\
% i.PE $\leftarrow$ PE /* Assign \textit{task-i} to the predicted PE */
\tcc{\textbf{Assign T to the predicted PE}}
}
\end{algorithm}

